Digging Deep into the layers of CNNs: In Search of How CNNs Achieve View Invariance

This paper is focused on studying the view-manifold structure in the feature spaces implied by the different layers of Convolutional Neural Networks (CNN). There are several questions that this paper aims to answer: Does the learned CNN representation achieve viewpoint invariance? How does it achieve viewpoint invariance? Is it achieved by collapsing the view manifolds, or separating them while preserving them? At which layer is view invariance achieved? How can the structure of the view manifold at each layer of a deep convolutional neural network be quantified experimentally? How does fine-tuning of a pre-trained CNN on a multi-view dataset affect the representation at each layer of the network? In order to answer these questions we propose a methodology to quantify the deformation and degeneracy of view manifolds in CNN layers. We apply this methodology and report interesting results in this paper that answer the aforementioned questions.

==> DP1_MORE_MEASURES.tex <==
\label{sec:moreMeaurements}
%\subsection{More Measurements}

As promised in the main paper, we define and show the results of more measurements such as KPLS-Norm Ratio and TPS-nonPolynomial. We use here the same notations and definitions stated in Section 4 in the main paper.
%To define these new measurements, we need to recall the following from the main paper. Let us denote the input data (images taken from a viewing circle and their pose labels) for of a specific object instance  as $\{(x_i \in \mathbb{R}^D , \theta_i \in [0,2 \pi] ) , i=1 \cdots N \}$, where $D$ denotes the dimensionality of the input image to the network, and $N$ is the number of the images, which are equally spaced around the viewing circle. These images form the view manifold of that object in the input space denoted by $\mathcal{M}=\{x_i\}_1^N$. Applying each image to the network will result in a series of linear and nonlinear transformations. Let us denote the transformation from the input to layer $l$ by the function $f_l(x):  \mathbb{R}^D \rightarrow {R}^{d_l} $ where $d_l$ is the dimensionality of the feature space of layer $l$.  With an abuse of notation we also denote the transformation that happens to the manifold $\mathcal{M}$ at layer $l$ by $\mathcal{M}^l=f_l(\mathcal{M})= \{ f_l(x_i)\}_1^N $. 
%After centering the data by subtracting the mean, let $\mathbf{A}^l=[\acute{f}_l(x_i) \cdots \acute{f}_l(x_N)]$ be the centered feature matrix at layer $l$ of dimension $d_l \times N$, which corresponds to the centered transformed images of the given object. We call $\mathbf{A}^l$ the sample matrix in layer $l$.

% data centering

%Since the dimensionality $d_l$ of the feature space of each layer varies, we need factor out the effect of the dimensionality. Since $N \ll l_d$ the transformed images on all the layers lie on  subspaces of dimension $N$ in each of the feature spaces.   Therefore we can change the bases to describe the samples using $N$ dimensional subspace \ie, we define the $N\times N$ matrices $\mathbf{\hat{A}}^l = \mathbf{U}^\textsf{T} \mathbf{A} $ where  $\mathbf{U} \in \mathbb{R}^{d_l \times N}$ are the orthonormal bases spanning the column space of $\mathbf{A}^l$ (which we can get by SVD of $\mathbf{A}^l=  \mathbf{U} \mathbf{S} \mathbf{V}^\textsf{T} $). This projection just rotate the samples at each layer, and it preserves the manifold properties. 

%All measures are evaluated per single view-manifold, which is represented by the $N$ transformed images. Let $v_i$ be the measurement value of the $i$th manifold. The overall score for every feature space/CNN layer is the mean over all view-manifolds i.e., $Score_{layer}=mean_i(v_i)$.


%\noindent{\bf Subspace Geometric Measurements:}


%\medskip
%\noindent{\em 1) Measure of spread - Nuclear Norm:} 
%%This is a measure of the spread of the data in the feature space of each layer. 
%There are several possible measures of the spread of the data in the sample matrix of each view manifold. We use the nuclear norm (also known as the trace norm~\cite{HornMatrixAnalysisBook}) defined as $|| \mathbf{A} ||_* = Tr (\sqrt{\mathbf{A}^\textsf{T}\mathbf{A}}) = \sum_{i=1}^N \sigma_i$, \ie it measure the sum of the singular values of  $\mathbf{A}$. 
%%\begin{equation}
%%   || \mathbf{A} ||_* = Tr (\sqrt{\mathbf{A}^\textsf{T}\mathbf{A}}) = \sum_{i=1}^N \sigma_i
%%\end{equation}
%Figure~\ref{SV_sum} shows that the nuclear norm of the transformed view manifolds in Model0 is almost monotonically decreasing as we go higher in the network, which indicates the the view manifolds is more spread in the lower layers. In fact at the output layer of Model0 the nuclear norm becomes too small, which indicates that the view manifold  is collapsing to reach view invariant representation at this layer.
%
%\medskip
%\noindent {\em 2) Subspace dimensionality measure - Effective-p:} As a measure of the effective dimensionality of the subspace where the view manifold lives, we define {\em Effective-p} as the minimum number of singular values (in decreasing order) that sum up to more that or equal to $p\%$ of the nuclear norm, 
%\begin{equation}
%  \text{Effetive}-p = \sup \{n: {\sum_{i=1}^n \sigma_i}/{\sum_{i=1}^N \sigma_i} \leq p/100 \}
%\end{equation} 
%A smaller number means that the view manifold samples live in a lower dimensional subspace. Figure~\ref{EffectiveSV90} ($p=90\%)$ shows that subspace dimension is  varying within a small range in the lower layers and it reduces dramatically in the fully connected layer, which also indicate the network is trying to achieve view invariant, where the minimum is achieved at the FC8 (even without fine tuning).  
%  
%\medskip  
%\noindent{\em 3) Alignment Measure -  KTA:}
%Ideally the view manifold resulting of the view sitting is a one-dimensional closed curve in the feature space, which can be thought as a deformed circle~\cite{zhang_aaai_2013}. This manifold can be degenerate in the ultimate case to a single point in case of a textureless object.  The goal of this measurement is to quantify how the transformed manifold locally preserves the original manifold structure. To this end we compare the kernel matrix of the transformed manifold at layer $l$, denote by $\mathbf{K}^l_n$, with the kernel matrix of the an embedding of the ideal view manifold on unit circle, denote by $\mathbf{K}_n^\circ$, where $n$ indicates the local neighborhood size used in constructing the kernel matrix. We construct the neighborhood based on the pose labels. 
%
%Given these two kernel matrices we can define several convergence measures.  We use {\em Kernel Target Alignment (KTA)} which has been used in the literature for kernel learning~\cite{Kandola_spectralkernel_2001}. It simply finds a scale invariant dependency between two normalized kernel matrices\footnote{We also experimented with HSIC~\cite{gretton2005measuring}, however HSIC is not scale invariant and is not designed to compare data in different feature spaces. Even after scaling the data, HSIC did not give any discriminative signal}. Therefore ,we define the alignment of the transformed view manifold $\mathcal{M}^l$ at layer $l$  with the ideal manifold as
%\begin{equation}
%  KTA_n(\mathcal{M}^l) =  \frac{<\mathbf{K}_n^l,\mathbf{K}_n^\circ>_F}{|| \mathbf{K}_n^l,||_F  || \mathbf{K}_n^\circ ||_F }
%\end{equation}
%Figure~\ref{kta} shows the KTA applied to Model0, where the we can notice that the alignment is almost similar across the lower layers, with Pool5 having the maximum alignment, and then starts to drop at the very high layers. which indicates that after Pool5, the FC layers try to achieve view invariant. It is justifiable that Pool5 has better alignment than the lower layers, since the lower layers will not be translation invariant as Pool5.


%\noindent{\em 6)  Hilbert-Schmidt Independence Criterion (HSIC) \cite{Gretton_2005}:  is a convergence measure between two kernels (affinity matrices). We use HSIC to measures the correlation between the two sets of points (the set of points on the view-manifold and set of points on the circle) based on the spatial structure of the points in each set, by measuring how far they are both extracted from the same distribution. 
%%\textit{\textbf{old description:} how far the two set of points (the set of points on the view-manifold and set of points on the circle) are extracted from the same distribution $p_z$ the similarity(dependence) between the data affinity matrix and the affinity matrix of the points on the unit circle. This measure the global Euclidean structure of the datapoints compared to the Euclidean structure of the corresponding points on the unit circle. }
%Empirically HSIC is approximated by
%
%\[HSIC(A,B) = \frac{1}{(n-1)^2}trace(A*H*B*H)\]
%
%Where $A$ and $B$ are two affinity matrices, $H = I_n - \frac{1}{(n)} \mathbf{1}_{n\times n}$, $\textbf{I}$ is the unit matrix and $\mathbf{1}$ is matrix of all ones. The matrix $H$ centerlizes the data in the feature space.

\medskip
\noindent{\em 1) KPLS-Norm Ratio:}  
Kernel Partial Least Squares (KPLS) \cite{Rosipal_kpls_2002} is a supervised regression method. KPLS iteratively extracts a set of principal components of the input kernel that are most correlated with the output. 
While KPCA extracts the principal components (PCs) of the kernel of the input data to maximize the variance of the output space, KPLS extracts the PCs of the kernel of the input data that maximize the correlation with the output data.
We use KPLS to map the affinity matrix of the transformed view-manifold  ({\em view-kernel}) to the circle affinity matrix ({\em circle-kernel}). Following the convention of the main paper, let the view-kernel is denoted by  $\mathbf{K}^l$, and the circle-kernel is denoted by $\mathbf{K}^\circ$ ({\em The subscript $n$ is removed to simplify the notation}).
We limit the number of extracted PCs to $d$ , where $d\ll N$ and $N$ is the dimensionality of the input kernel (in this work, we use $d=5$).
More specifically, KPLS maps the rows of $\mathbf{K}^l$ to the rows of $\mathbf{K}^\circ$. So that
\begin{equation}
\label{eq:kpls_regression}
\hat{\mathbf{K}}^\circ= \mathbf{G_0U}(\mathbf{T^\top G_0U})^{-1}\mathbf{T}^\top \mathbf{K}^l
\end{equation}
Where the set of extracted PCs are the columns of the matrix $T_{N\times d}$, $U_{N\times d}$ is auxiliary matrix, and the Gram-matrix $\mathbf{G_0}$ is defined by
\begin{equation}
\mathbf{G}_0= \frac{{\mathbf{K}^l} {\mathbf{K}^l}^\top}{b b^\top}
\label{eq:G_0}
\end{equation}
Where $b\in \mathbb{R}^N$ % is a $N$-Dim vector
, so that $b(i)$ is the Frobenius norm of the $i$-th row of $\mathbf{K}^l$. 
Based on the mapping in Eq~\ref{eq:kpls_regression}, we extract two measurements: 

First: {\em KPLS-Regression Error ($\delta$)} which measures geometric deformation of the generated output image of view-kernel in the circle-kernel space ($\hat{\mathbf{K}}^\circ$ with respect to the the circle-kernel (${\mathbf{K}}^\circ$) and the ). One choice for measuring this is
\[\delta(\hat{\mathbf{K}}^\circ , {\mathbf{K}}^\circ) = 1- KTA(\hat{\mathbf{K}}^\circ , {\mathbf{K}}^\circ) \]
Where KTA stands for Kernel Target Alignment (stated in Equation $2$ in the main paper).
%\frac{trac{\hat{\mathbf{K}}^\circ^\top }}{den}
The Regression error measures the reconstruction error of the circle-kernel from the view-kernel.
%
%mapping correctness from the view-kernel to the circle-kernel.

Second, KPLS-NormK Ratio ($\frac{\|G_d\|_{F}}{\|G_0\|_{F}}$) measure the residual energy after extracting the first $d$-PC's. Where $G_d$ is the residual of $G_0$ after $d$-iterations. %is the gram matrix of the rows of the view-kernel, and $k$ is the residual gram matrix after extracting $d$-PC's. 
The intuition behind this measure is that the larger the ratio $\frac{\|G_d\|_{F}}{\|G_0\|_{F}}$, this means that the view-manifold has more than $d$-PC's correlated with the circle-kernel. 

While KPLS-regression Error is self-explanatory (this measure presented in the main paper), using the two KPLS measurements together gives more precise view on the correlation between the view-manifold and the circle-manifold. 
From Fig~\ref{normk_ratio}, KPLS-Norm Ratio supports the observation that we noted in the main paper, from Fig~\ref{regression_err}, that the lower layers in Model0 are more correlated to the circle-manifold than the higher layers. Except for Pool5, which encodes maximum correlation between the view-manifold and the circle-manifold. %, where Pool5 has the least error. In general the lower layers has less error. This indicates that the lower layers preserve higher correlation with the ideal manifold structure.

%First:  {\em KPLS-Norm Ratio} $=\frac{||k||_F}{Norm(||k_0||_F)}$, which  measures the relative residual of the input kernel after extracting the first $d$-PC's. The intuition is that larger ratio  means that the view-manifold has more than $d$-PC's correlated with the circle manifold.

%Second:  These two scores are complementary to measure the correlation between the transformed view-manifold kernel and its corresponding circle kernel.


\medskip
\noindent{\em 2) TPS-nonlinearity measure:} 
In this measure we learn a regularized Thin Plate Spline (TPS) non-linear mapping~\cite{duchon1977splines} between the unit circle manifold and each manifold $\mathcal{M}^k$. 
The mapping function ($\gamma$) can be written as
\[\gamma^k(\mathbf{x}) = \mathbf{C}^k  \cdot \psi(\mathbf{x}),\]
where $\mathbf{C}_{d \times (N+e+1)}$ is the mapping matrix, $e=2$, and 
%a $$-dimensional mapping matrix with the $l$-th row $[\omega^l_1, \cdots, \omega^l_M, {c^l}^T]$. 
the vector $\psi(x)=[\phi(|x-z_1|) \cdots \phi(|x-z_M|),1,x^T]^T$  represents a nonlinear kernel map from the  conceptual representation to a kernel induced space. The thin plate spline is defined as: $\phi(r) = r^3$ and $\{z_i\}_{i=1}^{M}$ are the set of center points. The solution for $\mathbf{C}^k$ can be obtained by directly solving the linear system:
%\vspace{-2px}
\begin{equation}
\small
\begin{pmatrix} \mathbf{K}^l+\lambda \mathbf{I} & \mathbf{P}_x \\
 \mathbf{P}_t^T & \mathbf{0}_{(e+1) \times (e+1) } \end{pmatrix}_k  {\mathbf{C}^k}^T= \begin{pmatrix} \mathbf{A}_k \\ \mathbf{0}_{(e+1) \times d} \end{pmatrix},
\end{equation}
$\mathbf{A}$, $\mathbf{P}_x$ and $\mathbf{P}_t$ are defined for the $k-th$ set of object images as: $\mathbf{A}$ is a $N_k \times M$ matrix with $\mathbf{K}^l_{ij}=\phi(|x^k_i - z_j|), i=1,\cdots,N_k, j=1,\cdots,M, \mathbf{P}_x$ is a $N_k \times (e+1)$ matrix with $i$-th row $[1,\mathbf{x}^{k^T}_i]$, $\mathbf{P}_t$ is $M \times (e+1)$  matrix with $i$-th row $[1,\mathbf{z}^T_i]$. $A_k$ is a $N_k \times d$ matrix containing the set of images for manifold $\mathcal{M}^k$, \emph{i.e.} $\mathbf{A}_k=[\mathbf{y}_1^k,\cdots, \mathbf{y}^k_{N_k}]$. Solution for $\mathbf{C}^k$ is guaranteed under certain conditions on the basic functions used.

The reason for using TPS in particular is that the mapping has two parts, an affine part (linear polynomial) and a nonlinear part. Inquiring into the two parts gives an impression about the mapping, if it is mostly linear or nonlinear. We used the {\em reciprocal-condition number (RCond)} of the submatrices of the coefficient matrix that correspond to the affine and the nonlinear part. 

While Fig~\ref{tps_poly} shows that the lower layers has more (better) conditioned linear mapping.  Fig~\ref{tps_cf} shows that the lower layer has complete stable mapping. This is expected since the lower layers have high dimensionality. At the same time, Fig~\ref{tps_cf} shows that the Convolution layers (Conv 3,4 and 5) have unstable nonlinear mappings. An additional observation is that fine-tuning against the pose labels increases the mapping stability (polynomial and non-polynomial). It is clear in Fig~\ref{tps_cf} that the $TPS-RCond(CF-nonPoly)$ has very small order of values ($10^{-11}$), therefore, we do not rely on it in our analysis.

%this is a form of Generalized Radial Basis Function (GRBF) \cite{grbf}. Typical choices for the basis function include thin-plate spline, multiquadric, Gaussian\footnote{A Gaussian kernel does not need a polynomial part}, biharmonic and tri-harmonic splines. 
%\vspace{-2px}
%To ensure orthogonality and to make the problem well posed, the following condition constraints are imposed:  $\Sigma^M_{i=1} \omega_i p_j(x_i) = 0, j=1,\cdots,m$, where $p_j$  are the linear basis of $p$. Therefore, 


%\medskip
%\noindent{\bf Evaluation Measures:}
%We also evaluate the feature spaces at each layer by three empirical evaluation measures. For a test image $x$ transformed to the $l$-th layer feature space $f_l(x)$, we compute the performance of three classifiers (based on mapping the training data to the same feature space through $f_l(\cdot)$): {1) \em Kernel Ridge Regression for Pose},   {2) \em Linear SVM Classifier for Category}, and 3) {\em KNN classifier for pose and category}. 

\begin{figure}[h!]
\centering
%\begin{subfigure}[b]{0.32\columnwidth}
%  \caption{\scriptsize $\sum SV's$}
%  \centering
%    \includegraphics[width=\textwidth,height=0.75\textwidth]{figs/AllModels-SV-Sum}
%        \label{SV_sum}
%\end{subfigure} 
%\begin{subfigure}[b]{0.32\columnwidth}
%  \caption{\scriptsize Effective $90\%$ SV's}
%  \centering
%    \includegraphics[width=\textwidth]{figs/AllModels-Z-EffectiveSV90}
%        \label{EffectiveSV90}
%\end{subfigure} 
%\begin{subfigure}[b]{0.32\columnwidth}
%  \caption{\scriptsize HSIC}
%  \centering
%    \includegraphics[width=\textwidth]{figs/AllModels-HSIC}
%    \label{hsic}
%\end{subfigure} 
%\begin{subfigure}[b]{0.32\columnwidth}
%  \caption{\scriptsize KTA}
%  \centering
%    \includegraphics[width=\textwidth]{figs/AllModels-KTA}
%    \label{kta}
%\end{subfigure}

\begin{subfigure}[b]{0.40\columnwidth}
  \caption{\scriptsize KPLS-Regression Error ($\delta$)}
  \centering
    \includegraphics[width=\textwidth, height=.85\textwidth]{figs/ThreeModels-KPLS-Kernel-Regressionerror}
    \label{regression_err}
\end{subfigure}
\begin{subfigure}[b]{0.40\columnwidth}
  \caption{\scriptsize KPLS-Norm Ratio ($\frac{norm(G_d)}{norm(G_0)}$)}
  \centering
    \includegraphics[width=\textwidth, height=.85\textwidth]{figs/ThreeModels-KPLS-Kernel-NormKratio}
    \label{normk_ratio}
\end{subfigure}
\begin{subfigure}[b]{0.40\columnwidth}
  \caption{\scriptsize TPS-$RCond(CF-poly)$}
  \centering
    \includegraphics[width=\textwidth, height=.85\textwidth]{figs/ThreeModels-TPS-RCondCF-poly}
    \label{tps_poly}
\end{subfigure}
\begin{subfigure}[b]{0.40\columnwidth}
  \caption{\scriptsize TPS-$RCond(CF-nonPoly)$}
  \centering
    \includegraphics[width=\textwidth,height=0.85\textwidth]{figs/ThreeModels-TPS-RCondCF-nonPoly}
    \label{tps_cf}
\end{subfigure}


\caption{Measurement analysis for the view-manifold in RGBD dataset based on features extracted from different layers of several CNN models. Every figure shows single measurement. Multiple lines is for different CNN model. X-axis is labeled by the layers.}
\end{figure}


==> DP1_pretrained_analysis_-_01052016.tex <==
%!TEX root = DP1-main.tex
\subsection{Instance View Manifold Analysis}

Figure \ref{F:AnalysisPlots2} shows the application of the instance-specific view manifold measurements on the images of the RGBD dataset when applied to a pre-trained network (Model0  - no fine-tuning).  This gives us an insight on the transformation that happens to the view manifold of each object instance at each layer of the network. Figure~\ref{SV_sum1} shows that the nuclear norm of the transformed view manifolds in Model0 is almost monotonically decreasing as we go higher in the network, which indicates that the view manifolds is more spread in the lower layers. In fact at the output layer of Model0 the nuclear norm becomes too small, which indicates that the view manifold  is collapsing to reach view invariant representation at this layer. Figure ~\ref{EffectiveSV901} ($p=90\%)$ shows that subspace dimension varies within a small range in the lower layers and it reduces dramatically in fully connected layers, which indicates that the network tries to achieve view invariance. The minimum is achieved at FC8 (even without fine tuning).   Figure~\ref{kta1} shows the KTA applied to Model0, where we can notice that the alignment is almost similar across the lower layers, with Pool5 having the maximum alignment, and then starts to drop at the very high layers. which indicates that after Pool5, the FC layers try to achieve view invariant. Fig~\ref{regression_err1} shows that KPLS regression error on Model0 dramatically reduces from FC8 down to Pool5, where Pool5 has the least error. In general the lower layers have less error. This indicates that the lower layers preserve higher correlation with the ideal manifold structure. Fig~\ref{tps_poly1} shows that the mapping is highly linear, which is expected because of the high dimensionality of the feature spaces. From Fig~\ref{tps_poly1} we can clearly notice that the lower layers has more better-conditioned linear mapping (plots for the nonlinear part is in Appendix~\ref{sec:moreAnalysisMultiviewDataset}.)%, which shows very small values ($\approx 10^{-11}$) compared to the linear part }.  

\begin{figure}[th!] %[ht!]
%\begin{wrapfigure}{R}{0.6\textwidth}
\centering
\begin{subfigure}[b]{0.35\hsize}
  \caption{\scriptsize Nuclear Norm}
  \centering
    \includegraphics[width=\textwidth,height=.6\textwidth]{__ThreeModels-SV-Sum.png}
        \label{SV_sum1}
\end{subfigure} 
\hspace{-1.5em}
\begin{subfigure}[b]{.35\hsize}
  \caption{\scriptsize Effective $90\%$ SV's}
  \centering
    \includegraphics[width=\textwidth,height=.6\textwidth]{__ThreeModels-Z-EffectiveSV90.png}
        \label{EffectiveSV901}
\end{subfigure}
\hspace{-1.5em} 
\begin{subfigure}[b]{0.35\hsize}
  \caption{\scriptsize KTA}
  \centering
    \includegraphics[width=\textwidth,height=.6\textwidth]{__ThreeModels-KTA.png}
    \label{kta1}
\end{subfigure}
%\begin{subfigure}[b]{0.19\textwidth}
%  \caption{\scriptsize KPLS-$\frac{norm(K)}{norm(K_0)}$}
%  \centering
%    \includegraphics[width=\textwidth]{figs/AllModels-KPLS-Kernel-NormKratio}
%    \label{normk_ratio}
%\end{subfigure}
\vspace{-1.5em}
\begin{subfigure}[b]{0.35\hsize}
  \caption{\scriptsize KPLS-Reg err}
  \centering
    \includegraphics[width=\textwidth,height=.6\textwidth]{__ThreeModels-KPLS-Kernel-Regressionerror.png}
    \label{regression_err1}
\end{subfigure}
\hspace{-1.5em}
\begin{subfigure}[b]{0.35\hsize}
  \caption{\scriptsize TPS-$RCond(poly)$}
  \centering
    \includegraphics[width=\textwidth,height=.6\textwidth]{__ThreeModels-TPS-RCondCF-poly.png}
    \label{tps_poly1}
\end{subfigure}
\caption{\footnotesize Measurement analysis for the view-manifold in RGBD dataset based on features extracted from different layers of several CNN models. Every figure shows single measurement. Multiple lines is for different CNN model. X-axis is labeled by the layers.\textit{Larger version of all figures in Appendix~\ref{sec:largerFigures}.}}
\label{F:AnalysisPlots2}
\end{figure}

From these measurements we can conclude:
%\begin{enumerate}[
% \setlength{\itemsep}{0pt}
% \setlength{\parskip}{0pt}
% \setlength{\parsep}{0pt}
%\item 
(1) The lower layers preserve the view manifolds. The manifolds start to collapse in the FC layers to achieve view invariance. Preserving the view manifold at the lower layers  is intuitive because of the nature of the convolutional layers. (2) The manifold at Pool5 achieves the best alignment with the pose labels. This is a less intuitive result; why does the representation after successive convolutions and pooling improves the view manifold alignment? even without seeing any dense view manifold in training, and even without any pose labels being involved in the loss.   The hypotheses we have to justify that Pool5 has better alignment than the lower layers is that Pool5 has better  translation invariant properties, which results in improvement of the view manifold alignment. 

%\end{enumerate}

\subsection{Global Object-View Manifold Analysis}

%\begin{wrapfigure}[th!]
\begin{wrapfigure}{R}{0.6\textwidth}
\centering
\begin{subfigure}[b]{0.51\hsize}
  \caption{\scriptsize Linear SVM}
  \centering
    \includegraphics[width=\textwidth,height=.6\textwidth]{plot_paper1_category2.png}
      %  \label{SV_sum1}
\end{subfigure} 
\hspace{-1.5em}
\begin{subfigure}[b]{0.51\hsize}
  \caption{\scriptsize Pose regression}
  \centering
    \includegraphics[width=\textwidth,height=.6\textwidth]{plot_paper1_pose_withcat.png}
      %  \label{SV_sum1}
\end{subfigure} 
\begin{subfigure}[b]{0.51\hsize}
  \caption{\scriptsize KNN for categorization}
  \centering
    \includegraphics[width=\textwidth,height=.6\textwidth]{model0_cat_KNN_dist2-RGBD.png}
      %  \label{SV_sum1}
\end{subfigure} 
\hspace{-1.5em}
\begin{subfigure}[b]{0.51\hsize}
  \caption{\scriptsize KNN for pose estimation}
  \centering
    \includegraphics[width=\textwidth,height=.6\textwidth]{model0_pose_KNN_dist2-RGBD.png}
       % \label{SV_sum1}
\end{subfigure} 
	    % \footnotesize   \includegraphics[width=0.49\columnwidth]{figs/plot_pose.png}
%\caption{\small Top-Left: the performance of linear SVM category classification over the layers of different model. Top-Right: the performance of pose regression over the layers of different models. Bottom-Left: KNN categorization. Bottom-right: KNN pose estimation.}
\caption{\footnotesize Categorization and pose estimation over the layers of different models.}% \textit{Larger version of all figures in Appendix~\ref{sec:largerFigures}.}}

\label{fig:SVMRidge1}
\end{wrapfigure}
The performance of Linear SVM and Kernel Regression is shown in Figure~\ref{fig:SVMRidge1}, using RGBD dataset (plots for Pascal3D are in Appendix~\ref{sec:moreAnalysisMultiviewDataset}). The figure clearly shows the conflict in the representation of the pre-trained network (categorization increases and pose estimation decreases). Linear separability of category is almost monotonically increasing up to FC6.  Linear separability in  FC7 and FC8 is worse, which is expected as they are task specific (no fine-tuning). Surprisingly Pool1 features perform very bad, despite being the most general features (typically they show Gabor like features and color blobs). In contrast, for pose estimation, the performance increases as we go lower in the network up to Conv4 and then slightly decreases. This confirms our hypothesis that lower layers offer better feature encoding for pose estimation. It seems that Pool5 provides feature encoding that offer the best compromise in performance, which indicates that it is the best in compromising between the linear separation of categories and the preservation of the view-manifold structure. 

What is surprising is that the pose estimation results do not drop dramatically in FC6 and FC7. We can still estimate the pose (with accuracy around 63\%) from the representation at these layers, even without any training on pose labels. This highly suggests that the network preserves the view manifold structure to some degree. For examples taking the accuracy as probability at layer FC6, we can vaguely conclude that 90\% of the manifolds are linearly separable and 65\% are pose preserved (we are somewhere between hypotheses 1 and 2 at this layer). 

The aforementioned conclusion is also confirmed by the KNN analysis. Very high accuracy is achieved using KNN for category and pose. The category gap is reducing as we go up in the network up to FC7 (almost 0 gap at FC6 and FC7).  In contrast the gap is large at all layers for pose estimation. This indicates separation of the  instances' view manifolds where the individual manifolds are not collapsed (This is why as we increase the neighborhood, the category performance stays the same while pose estimation decreases smoothly - See the top-right block of Figure~\ref{F:KNN}-right for illustration). The results above consistently imply that the higher layers of CNN (expect FC8 which is task specific), even without any fine-tuning on the dataset, and even without any pose label optimization achieve representations that separate and highly preserve the view manifold structure. 

%Tables \ref{tab1_rgbd} and \ref{tab2_pascal} show the quantitative results of our models, compared to baselines, on the RGBD Dataset and Pascal3D+. Table \ref{tab2_pascal} shows our quantitative results compared against two previous methods \citep{zhang2015factorization} and \citep{xiang_pascal3d_2014}, using the two metrics $<45^\circ$ and $<22.5^\circ$ \footnote{Pose accuracy metrics are defined in \citep{zhang2015factorization,xiang_pascal3d_2014} and stated in Appendix~\ref{sec:metrics_pose}}. It is important to note that the comparison with \citep{xiang_pascal3d_2014} is unfair because they solve for detection and pose simultaneously while we solve for categorization and pose estimation. Model1 here outperforms both \citep{zhang2015factorization} and \citep{xiang_pascal3d_2014} (despite the unfair comparison with the latter approach).
Table \ref{tab2_pascal} shows the quantitative results of our models on Pascal3D+ dataset. It also shows comparison against two previous methods \citep{zhang2015factorization} and \citep{xiang_pascal3d_2014}, using the two metrics $<45^\circ$ and $<22.5^\circ$ \footnote{Pose accuracy metrics are defined in \citep{zhang2015factorization,xiang_pascal3d_2014} and stated in Appendix~\ref{sec:metrics_pose}}. It is important to note that the comparison with \citep{xiang_pascal3d_2014} is unfair because they solve for detection and pose simultaneously while we solve for categorization and pose estimation. Model1 here outperforms both baselines (despite the unfair comparison with the latter approach). Quantitative results on RGBD dataset is presented in Appendix~\ref{sec:quant_rgbd}.

%Model1 here outperforms both \citep{zhang2015factorization} and \citep{xiang_pascal3d_2014} (despite the unfair comparison with the latter approach).

%\begin{table}
%	\scriptsize
%	\centering
%	\begin{tabular}{|l|c|c|}
%		\hline 
%		\textbf{Approach} & \textbf{Categorization} $\%$ & \textbf{Pose} $\%$ \\ 
%		\hline 
%		HOG (SVM/Kernel Regression) & 80.26 & 27.95 (AAAI) \\ 
%		\hline 
%		Model0 (SVM/Kernel Regression) on conv4 & 58.64 & 67.39 (AAAI)\\ 
%		\hline 
%		Model0 (SVM/Kernel Regression) on FC6 & 86.71 & 64.39 (AAAI) \\ 
%		\hline 
%		Model1 & 89.63 & 81.21 (AAAI), 69.58 ($<$ 22.5), 81.09 ($<$ 45) \\ 
%		\hline 
%	\end{tabular} 
%	\caption{\footnotesize RGBD Dataset Results for HOG, Model0 and Model1.}
%	\label{tab1_rgbd}
%\end{table}


\begin{table}[th!]
\centering
\scriptsize
\begin{tabular}{|l|c|c|c|} 
\hline
\textbf{Approach} & \textbf{Categorization  $\%$} &\textbf{Pose (AAAI metric $\%$)}& \textbf{Pose (other metrics $\%$)}\\ 
\hline 
{\textit{Model0 (SVM/Kernel Regression)}} &FC6/FC7/FC8 & FC6/FC7/FC8&\\
 & 73.64/76.38/71.13 & 49.72/48.24/45.41 &\\ 
\hline 
%{\textit{Model1 (SVM/Kernel Regression)}} & & &\\
%FC6/FC7/FC8 & 74.65/79.25/84.12 & 54.41/54.07/60.31 &\\ 
%\hline 
%{\textit{Model0 NN}} & & &\\
%FC6/FC7/FC8 & 60.05/69.89/61.26 & 61.11/61.38/60.32 &\\ 
%\hline 
%{\textit{Model1 NN}} & & &\\
%FC6/FC7/FC8& 73.50/77.30/83.07 & 65.87/66.07/70.54 &\\ 
{\textit{Model1 (SVM/Kernel Regression)}} & 74.65/79.25/84.12 & 54.41/54.07/60.31 &\\ 
\hline 
{\textit{Model0 NN}} & 60.05/69.89/61.26 & 61.11/61.38/60.32 &\\ 
\hline 
{\textit{Model1 NN}} & 73.50/77.30/83.07 & 65.87/66.07/70.54 &\\ 
\hline 
{\textit{Model1} (final prediction)} &  84.00 &   71.60 & 47.34($<$22.5), 61.30 ($<$45)  \\ \hline
% \multicolumn{3}{|c|}{\textit{State of the Art Methods}} \\ \hline
~\citep{zhang2015factorization} &  - & - & 44.20 ($<$ 22.5), 59.00 ($<$45) \\  \hline
~\citep{xiang_pascal3d_2014} & -  & - & 15.6  ($<$22.5), 18.7 ($<$45)\\ 
\hline
\end{tabular} 
\caption{\footnotesize Pascal3D Performance computed for Model0 and Model1 using different classification techniques. Comparsion indicates that Model1 outperforms the baselines. % from \citep{zhang2015factorization} and \citep{xiang_pascal3d_2014} using the two metrics $<45^\circ$ and $<22.5^\circ$. It is important to note that the comparison with \citep{xiang_pascal3d_2014} is slightly unfair because they solve for detection and pose simultaneously while we do not solve for detection. We solve for categorization and pose. 
%Model1 here outperforms both \citep{zhang2015factorization} and \citep{xiang_pascal3d_2014} (despite the unfair comparison with the latter approach).
}
\label{tab2_pascal}
\end{table}

%\begin{table}
%\centering
%\scriptsize
%\begin{tabular}{|l|c|c|} 
%\hline
%\textbf{Approach} & \textbf{Categorization  \%} &\textbf{Pose (AAAI metric)}\\ 
%\hline 
%\multicolumn{3}{|c|}{\textit{Model0 (SVM/Kernel Regression)}} \\ 
%\hline 
%FC6/FC7/FC8 & 73.64/76.38/71.13 & 49.72/48.24/45.41 \\ 
%\hline 
%\multicolumn{3}{|c|}{\textit{Model1 (SVM/Kernel Regression)}} \\ 
%\hline 
%FC6/FC7/FC8 & 74.65/79.25/84.12 & 54.41/54.07/60.31 \\ 
%\hline 
%\multicolumn{3}{|c|}{\textit{Model0 NN}}\\  \hline
%FC6/FC7/FC8 & 60.05/69.89/61.26 & 61.11/61.38/60.32 \\ 
%\hline 
%\multicolumn{3}{|c|}{\textit{Model1 NN}} \\ \hline
%FC6/FC7/FC8& 73.50/77.30/83.07 & 65.87/66.07/70.54 \\ 
%\hline 
%\multicolumn{3}{|c|}{\textit{Model1 (direct prediction from CNN)}} \\ \hline
%output &  84.00 &   71.60 (AAAI), 47.34($<$22.5), 61.30 ($<$45)  \\ \hline
%\multicolumn{3}{|c|}{\textit{State of the Art Methods}} \\ \hline
%~\citep{zhang2015factorization} &  - & 44.20 ($<$ 22.5), 59.00 ($<$45) \\  \hline
%~\citep{xiang_pascal3d_2014} & -  &  15.6\% ($<$22.5), 18.7\% ($<$45)\\ 
%\hline
%\end{tabular} 
%\caption{Pascal3D Performance. Here we see our results compared to the two baselines from \citep{zhang2015factorization} and \citep{xiang_pascal3d_2014} using the two metrics $<45^\circ$ and $<22.5^\circ$. It is important to note that the comparison with \citep{xiang_pascal3d_2014} is slightly unfair because they solve for detection and pose simultaneously while we do not solve for detection. We solve for categorization and pose. Model1 here outperforms both \citep{zhang2015factorization} and \citep{xiang_pascal3d_2014} (despite the unfair comparison with the latter approach).}
%\label{tab2_pascal}
%\end{table}






==> DP1_probdef_-_New.tex <==
% !TEX root = DP1-main.tex

% Problem Definition for the manifold analysis paper

It is expected that multiple views of an object lie on intrinsically low-dimensional manifolds ({\emph view manifold}\footnote{we use the terms \textit{view manifold }and \textit{viewpoint manifold }interchangeably}) in the input space. View manifolds of different instances and different objects are spread out in this input space, and therefore form jointly what we call the {\emph object-view manifold}. The input space here denotes the $R^{N\times M}$ space induced by an input image of size $N \times M$, which is analogous to the retinal array in the biological system. For the case of a viewing circle(s), the view manifold of each object instance is expected to be a 1-dimensional closed curve in the input space. The recovery of the category and pose of a test image reduces to finding which of the manifolds this image belongs to, and what is the intrinsic coordinate of that image within that manifold. This view of the problem is shared among manifold-based approaches such as~\citep{murase95visual,zhang_aaai_2013,bakry_untangling_2014}

The ability of a vision system to recover the viewpoint is directly related to how the learned representation preserves the view manifold structure. If the transformation applied to the input space yields a representation that  results in collapsing the view manifold, the system will no longer be able to discriminate between different views. Since each layer of a deep NN re-represents the input in a new feature space, the question would be how the re-representations deform a manifold that already exists in the input space.  A deep NN would satisfy the hypothesis of \textit{'flattening'} and \textit{'untangling'} by ~\cite{dicarlo2007untangling}, if the representation in a given layer separates the view manifolds of different instances, without collapsing them, in a way to be able to put a separating hyperplanes between different categories. 
%% can be removed
\begin{wrapfigure}{R}{0.7\textwidth}
	%\begin{figure*}
	\vspace{-7mm}
	%\begin{minipage}{\hsize}
	%\centering
	%[width=1.0\linewidth]
	%  \includegraphics[natwidth=320bp,natheight=160bp,width=1.0\linewidth]{Four_hypotheses}%[width=3.2in, height=1.8in]{Four_hypotheses.png}
	\includegraphics[width=\hsize]{Four_hypotheses}
	\caption{\footnotesize Sketches of four hypotheses about possible structures of the view manifolds of two objects in a given feature space. %\textit{Larger version of all figures in Appendix~\ref{sec:largerFigures}.}
	}
	\label{F:Four_hypotheses}
	%\end{minipage}
\end{wrapfigure}
Typically CNN layers exhibit general-to-specific feature encoding, from Gabor-like features and color blobs at low layers to category-specific features at higher layers~\citep{fergus_visualizecnn_2013}. We can hypothesize that for the purpose of pose estimation, lower layers should hold more useful representations that might preserve the view manifold and be better for pose estimation. But which of these layers would be more useful, and where does the view-manifold collapse to view-invariance.

%\hspace{-1em}
There are different hypotheses we can make about how the view manifolds of different objects are arranged in the feature space of a given layer. These hypotheses are shown in Figure~\ref{F:Four_hypotheses}. We arrange these hypotheses based on linear separability of the different objects' view manifolds and the preservation of the view manifolds. Case 0 is the non-degenerate case where the visual manifolds preserve the pose information but are tangled and there is no linear separation between them (this might resemble the input space, similar to left case in Figure~\ref{DiCarloModel}). Case 1 is the ultimate case where the view manifolds of different objects are preserved by the transformation and are separable (similar to the right case in Figure~\ref{DiCarloModel}).  Case 2 is where the transformation in the network leads to separation of the object's view manifold at the expense of collapsing these manifolds to achieve view invariance. Collapsing of the manifolds can be to different degrees, to the point where each object's view manifold can be mapped to a single point. Case 3 is where the transformation results in more tangled manifolds (pose collapsing and non-separable). It is worth to notice that both cases 1 and 2 are view invariant representations. However, it is obvious that case 1 would be preferred since it also facilitates pose recovery. It is not obvious whether optimizing a network with a categorization loss result in case 1 or case 2. 
Getting an insight about which of these hypotheses are true in a given layer of a CNN is the goal of this paper. In Section~\ref{S:ManifoldAnalysis} we propose a methodology to get us to that insight.%

\subsection{Experimental Settings}
To get an insight into the representations of the different layers and answer the questions posed in Section~\ref{S:Intro} we experiment on two datasets: I) RGB-D dataset~\citep{lai2011large}, II) Pascal3D+ dataset~\citep{xiang_pascal3d_2014}. We selected the RGB-D dataset since it is the largest available multiview dataset with the most dense viewpoint sampling. The dataset contains 300 instances of tabletop objects (51 categories). Objects are set on a turntable and captured by an Xbox Kinect sensor (Kinect 2010) at 3 heights (30$^\circ$, 45$^\circ$ and 60$^\circ$ elevation angles). The dense view sampling along each height is essential for our study to guarantee good sampling of the view manifold. We ignore the depth channel and only used the RGB channels. 
\begin{wrapfigure}{R}{0.7\textwidth}
	%\begin{minipage}{\hsize}
	%	\centering
	\vspace{-7mm}
	%\includegraphics[width=\linewidth,height=0.6\linewidth]{KNNtradeoffs.png}%[width=2.8in, height=1.5in]{KNNtradeoffs.png}
	\includegraphics[width=\hsize]{KNNtradeoffs.png}
	\caption{\footnotesize KNN Tradeoffs: Left) accuracy tradeoff between pose and category estimation using KNN. Right).}% Gap tradeoff (Gap is the drop in performance as K increases.)}
	\label{F:KNN}
	%\end{minipage}
	\vspace{-4mm}
	%\end{figure*}
\end{wrapfigure}
Pascal3D+ is very challenging because it consists of images ``in the wild'', in other words, images of object categories exhibiting high variability, captured in uncontrolled settings and under many different poses. Pascal3D+ contains 12 categories of rigid objects selected from the PASCAL VOC 2012 dataset \citep{Pascal}. These objects are annotated with 3D pose information ({\emph{i.e}}, azimuth, elevation and distance to camera). Pascal3D+ also adds 3D annotated images of these 12 categories from the ImageNet dataset \citep{imNet09}. The {\it bottle} category is omitted in state-of-the-art results. This leaves 11 categories to experiment with. There are about 11,500 and 7,000 training images in ImageNet and Pascal3D+ subsets, respectively.  For testing, there are about 11,200 and 6,900 testing images for ImageNet and Pascal3D+, respectively. On average there are about 3,000 object instances per category in Pascal3D+, making it a challenging dataset for estimating object pose.

The two datasets provide different aspect of the analysis. While the RGB-D provides dense sampling of each instance's view manifold,  Pascal3D+ dataset contains only very sparse sampling.  Each instance is typically imaged from a single viewpoint, with multiple instances of the same category sampling the view manifold at arbitrary points.
 Therefore, in our analysis we use the RGB-D dataset to analyze each instance viewpoint manifold and the combined object-viewpoint manifolds, while the Pascal3D provides analysis of the viewpoint manifold at the category level.

\noindent{\bf Evaluation Split:}
For our study, we need to make sure that the objects we are dealing with have non-degenerate view manifolds. We observed that many of the objects in the RGB-D dataset are ill-posed, in the sense that the poses of the object are not distinct. This happens when the objects have no discriminating texture or shape to be able to identify the different poses (\emph{e.g.} a texture-less ball, apple or orange on a turntable). This will cause view manifold degeneracy. Therefore we select 34 out of the 51 categories as objects that possess pose variations across the viewpoints, and thus are not ill-posed with respect to pose estimation.

We split the data into training, validation and testing. Since in this datasets, most categories have few instances, we left out two random object instances per category, one for validation and one for testing. In the case where a category has less than 5 instances, we form the validation set for that category by randomly sampling from the training set. Besides the instance split, we also left out all the middle height for testing. Therefore, the testing set is composed of unseen instances and unseen heights and this allows us to more accurately  evaluate the capability of the CNN architectures in discriminating categories and estimating pose of tabletop objects. 
\subsection{Base Network: Model0}
%Description of the base network here.
The base network we use is the Convolutional Neural Network described in \cite{krizhevsky2012imagenet} and winner of LSVRC-2012 ImageNet challenge~\citep{li_imagenet_2014}. The CNN was composed of 8 layers (including 1000 neuron output layer corresponding to 1000 classes). We call these layers in order: Conv1, Pool1, Conv2, Pool2, Conv3, Conv4, Conv5, Pool5, FC6, FC7, FC8 where Pool indicates Max-Pooling layers, Conv indicates layers performing convolution on the previous layer and FC indicates fully connected layer. The last fully connected layer (FC8) is fed to a 1000-way softmax, which produces a distribution over the category labels of the dataset. 
%Dropout was employed during training.  Rectified Linear Units (ReLU) were used for faster training. 
%Data augmentation was conducted on the images and consisted of translations, horizontal reflections, Gaussian noise addition to the pixel intensities. 
%For training, stochastic gradient descent was employed. 
%Throughout this study we vary the architecture of this network and change the loss functions to study its behavior. We augment the training dataset in this study by randomly sampling 227x227 patches from the downscaled images of size 256x256. At test time the center 227x227 patches are taken.




==> moreAnalysisMultiviewDataset.tex <==
\section{Analysis using KNN Measure on Multiview Datasets}
\label{sec:moreAnalysisMultiviewDataset}
In this section we show KNN performance for Model1Cat and Model1Pose on the RGBD dataset for both pose estimation and categorization tasks (Figure~\ref{F:moreRGBD}). %\ref{fig:model1catrgbdcnn1} to \ref{fig:model1catrgbdcnn4}). 
We also analyze the performance of Model0, Model1Pose and Model1Cat on Pascal3D+ for both pose estimation and categorization tasks (Figure \ref{F:morePascal3D}).%\ref{fig:model1catrgbdcnn_pascal1} to \ref{fig:model1catrgbdcnn_pascal6}).

%\newpage

%\subsubsection{RGBD Dataset}
\begin{figure*}[ht!] %[ht!]
\begin{subfigure}[b]{0.49\textwidth}
	\centering
	\caption{Model1Cat: KNN on Categorization}
	\includegraphics[width=\textwidth,height=.8\textwidth]{model1CAT_cat_KNN_dist2.png}
	\label{fig:model1catrgbdcnn1}
	
\end{subfigure}
\begin{subfigure}[b]{0.49\textwidth}
	\centering
	\caption{Model1Cat: KNN on Pose Estimation}
	\includegraphics[width=\textwidth,height=.8\textwidth]{model1CAT_pose_KNN_dist2.png}
	\label{fig:model1catrgbdcnn2}
\end{subfigure}
\begin{subfigure}[b]{0.49\textwidth}
	\centering
	\caption{Model1Pose: KNN on Categorization}
	\includegraphics[width=\textwidth,height=.8\textwidth]{model1POSE_cat_KNN_dist2.png}

	\label{fig:model1catrgbdcnn3}
\end{subfigure}
\begin{subfigure}[b]{0.49\textwidth}
	\centering
	\caption{Model1Pose: KNN on Pose Estimation}
	\includegraphics[width=\textwidth,height=.8\textwidth]{model1POSE_pose_KNN_dist2.png}
	\label{fig:model1catrgbdcnn4}
\end{subfigure}
\caption{RGBD Dataset: KNN performace for Categorization and Pose Estimatoin applied on Model1Cat and Model1Pose}
\label{F:moreRGBD}
\end{figure*}

%\clearpage

%\subsubsection{Pascal3D Dataset}
\begin{figure*}[ht!] %[ht!]
\begin{subfigure}[b]{0.49\textwidth}
	\centering
	\caption{Model0: KNN on Categorization}
	\includegraphics[width=\textwidth,height=.7\textwidth]{model0cat_knn_pascal3D.png}
	\label{fig:model1catrgbdcnn_pascal1}
\end{subfigure}
\begin{subfigure}[b]{0.49\textwidth}
	\centering
	\caption{Model0: KNN on Pose Estimation}
	\includegraphics[width=\textwidth,height=.7\textwidth]{model0pose_knn_pascal3D.png}
	\label{fig:model1catrgbdcnn_pascal2}
\end{subfigure}
\begin{subfigure}[b]{0.49\textwidth}
	\centering
	\caption{ Model1Cat: KNN on Categorization}
	\includegraphics[width=\textwidth,height=.7\textwidth]{model1CAT_catknn_pascal3D.png}
	\label{fig:model1catrgbdcnn_pascal3}
\end{subfigure}
\begin{subfigure}[b]{0.49\textwidth}
	\centering
	\caption{Model1Cat: KNN on Pose Estimation}
	\includegraphics[width=\textwidth,height=.7\textwidth]{model1CAT_poseknn_pascal3D.png}
	\label{fig:model1catrgbdcnn_pascal4}
\end{subfigure}
\begin{subfigure}[b]{0.49\textwidth}
	\centering
	\caption{Model1Pose: KNN on Categorization}
	\includegraphics[width=\textwidth,height=.7\textwidth]{model1POSE_catknn_pascal3D.png}
	\label{fig:model1catrgbdcnn_pascal5}
\end{subfigure}
\begin{subfigure}[b]{0.49\textwidth}
	\centering
	\caption{Model1Pose: KNN on Pose Estimation}
	\includegraphics[width=\textwidth,height=.7\textwidth]{model1POSE_poseknn_pascal3D.png}
	\label{fig:model1catrgbdcnn_pascal6}
\end{subfigure}
\caption{Pascal 3D Dataset: KNN performace for Categorization and Pose Estimatoin applied on Model0, Model1Cat and Model1Pose}
\label{F:morePascal3D}
\end{figure*}
